A Framework to Manage the Complex Organisation of Collaborating: Its Application to Autonomous Systems

In this paper we present an analysis of the complexities of large group collaboration and its application to develop detailed requirements for collaboration schema for Autonomous Systems (AS). These requirements flow from our development of a framework for collaboration that provides a basis for designing, supporting and managing complex collaborative systems that can be applied and tested in various real world settings. We present the concepts of "collaborative flow" and "working as one" as descriptive expressions of what good collaborative teamwork can be in such scenarios. The paper considers the application of the framework within different scenarios and discuses the utility of the framework in modelling and supporting collaboration in complex organisational structures.

==> eptcsdata.tex <==
\providecommand{\event}{Jeremy W. Bryans and John S. Fitzgerald (Eds.): \\
Formal Aspects of Virtual Organisations 2009 (FAVO2009)}
\providecommand{\volume}{16}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{51}
\providecommand{\eid}{5}

